A Search Strategy and Vessel Detection in Maritime Environment Using Fixed-Wing UAVs

In this paper, we address the problem of autonomous search and vessel detection in an unknown GNSS-denied maritime environment with fixed-wing UAVs. The main challenge in such environments with limited localization, communication range, and the total number of UAVs and sensors is to implement an appropriate search strategy so that a target vessel can be detected as soon as possible. Thus we present informed and non-informed methods used to search the environment. The informed method relies on an obtained probabilistic map, while the non-informed method navigates the UAVs along predefined paths computed with respect to the environment. The vessel detection method is trained on synthetic data collected in the simulator with data annotation tools. Comparative experiments in simulation have shown that our combination of sensors, search methods and a vessel detection algorithm leads to a successful search for the target vessel in such challenging environments.

==> Content/extended_abstarct/1-introduction.tex <==
% Introduction + motivation
In a maritime environment, autonomous vehicles can be used for security, environmental monitoring, emergency operations such as search and rescue, or inspection of vessels and cargoes. Nowadays, poaching, smuggling, piracy, and human trafficking are becoming more common problems in such environments. Therefore, the security of maritime areas is of great importance.
Motivated by these problems ASPIRE \cite{ASPIRE}, the program management of Abu Dhabi's Advanced Technology Research Council, has organized the Mohamed Bin Zayed International Robotics Challenge (MBZIRC) 2023 \cite{MBZIRC}. The challenge aims to apply ground-breaking, state-of-the-art technologies to tackle the aforementioned problems. 
% The total prize money of the challenge in US is $ \$ 3,250,000$. 

The main idea of the challenge is to deploy a heterogeneous robotic system, composed of Unmanned Aerial Vehicles (UAVs), Unmanned Surface Vehicles (USVs) and a robotic arm attached to a USV, to collaboratively execute a mission consisting of inspection and intervention tasks. The inspection task consists of searching a given area and looking for a target vessel using UAVs, while the intervention task's goal is to approach the target vessel with a USV and pick up the required objects on the vessel with an UAV eqippped with a manipulator. To make the whole competition even more challenging, several restrictions were introduced, such as the impossibility to use the Global Navigation Satellite System (GNSS) for positioning and navigation. Another restriction was the availability of only short-range communication among robots \cite{MBZIRC}.

The first phase of the competition consisted of submitting a white paper. In the second phase, the task was to complete the mission described above in the given simulator.  Our team, University of Zagreb, Faculty of Electrical Engineering and Computing (UNIZG-FER), was selected as one of the semi-finalists to participate in the second phase. 
% The team has been divided into several subgroups addressing different subtasks.
This paper describes our team's approach and solution to the inspection task, while the same for the intervention task is described in \cite{Fausto}. 

As mentioned, the inspection task includes search and detection of the target vessel with fixed-wing or quadrotor UAVs. The search zone is defined as 10 $\mathrm {km}^2$ area over the sea. Due to the limited mission time (60 minutes) and a relatively large area to be covered, the fixed-wing UAVs are preferred over quadrotor UAVs. The fixed-wing UAVs are faster and frequently used for detection, coverage and search tasks. The provided model of fixed-wing UAV \cite{FW_book} is shown in Fig. \ref{fig:fw}.

\begin{figure}[t!]
 \centerline{\includegraphics[trim = {3cm 3cm 3cm 4cm}, clip, scale = 0.27]{images/zephyr.png}}
 \caption{A fixed-wing UAV flies in the search area above the vessel.}
 \label{fig:fw}
\end{figure}
 

==> Content/extended_abstarct/2-control.tex <==
 %control
For the given model of a fixed-wing UAV, the control inputs for the model in the simulator are roll, pitch and angular velocity of the propellers. Two uncoupled PID controllers are implemented to control the latitudinal and longitudinal motion of the UAV. The longitudinal motion is controlled by changing the pitch angle while the latitudinal motion (as well as yaw) is controlled by the roll angle.
The angular velocity of the propellers is used to set the velocity of the UAV. The relationship between the angular velocity of the propellers and the velocity of the UAV is determined experimentally by fitting the curve over a set of points. For the given angular velocity of the propellers, a simulation of the UAV is performed, while the ground velocity is calculated from the ground truth location data.
Please note that for simplicity, the presence of wind is neglected and the angle of sideslip and angle of attack are assumed to be zero. Therefore, several simplifications can be introduced \cite{FW_book}:
\begin{enumerate*}
    \item The airspeed is equal to the ground speed,
    \item The course angle is equal to the heading angle.
\end{enumerate*}

The fixed-wing UAVs are equipped with several sensors, such as IMU, magnetometer and barometer. Due to the good measurements of the barometer and accelerometer, as well as the attitude angles from IMU, the data is processed with a low pass filter before being used to estimate the horizontal position in the linear Kalman filter model. The barometer measurements are used to estimate the altitude. In addition to the standard sensors mentioned earlier, there is also a Radio Frequency (RF) range sensor and HD cameras mounted on the side and to the front of the UAV. The RF sensor obtains range measurements used in relative localization algorithm, while the HD cameras are used for target detection. The relative localization algorithm utilizes all available range measurements exchanged among the agents to localize the whole system relative to fixed base stations. The measurements obtained from the localization algorithm are used for correction in the Kalman filter.
To ensure that the UAV follows the given waypoints, the method with fillet transitions from \cite{FW_book} is used. In this way, instead of a usual sharp transition in the waypoint, the transition between two path segments is smoothed by defining the orbit. Furthermore, with this method, the UAV deviates less from the given path.

 \begin{figure}[t!]
 \centering
 \includegraphics[trim = {11cm 1cm 12cm 3cm}, clip,width=0.91\columnwidth]{images/lawn2.png}
 \caption{An example of a lawnmower over the smaller search area. The figure shows for each UAV its actual position (red), its estimated position (yellow) and the position provided by the localization module (green). The measurements from the RF sensors are within a radius of 1000 $m$ around the starting point.}
 \label{fig:lawn}
\end{figure}

In order to find the target vessel as quickly as possible, we focus on covering the area with a certain number of fixed-wing UAVs. Since the number of UAVs in the mission is limited \cite{MBZIRC}, our approach utilizes 3 fixed-wing UAVs responsible for 3 equal parts of the area. 
% In order to cover the entire area and search for the target vessel, 3 fixed wing are used and the whole area was divided into 3 equal parts. 
Recently, two search patterns are tested, spiral and lawnmower. Finally, the lawnmower pattern (Fig. \ref{fig:lawn}) is selected due to shorter coverage time.  

%Since UAVs were gradually moving further away from the starting gates, the %communication structure was able to easily follow it.
%\Todo{Add a sentence about communication}

==> Content/extended_abstarct/3-detection.tex <==
%detection
For the vessel detection YOLOv5 \cite{YOLOv5} is used. A model is trained to detect seven different types of vessels. Since the gimbal for the camera is not provided, the problem of rotating the camera frame is solved by data augmentation and extending the training set with rotated images of the vessels. Examples of detected vessels in the front camera view are shown in Fig. \ref{fig:Vess_example}. Besides the type of vessel, the global position is also calculated. It is determined by combining transformations and the relative position of the vessel with respect to the fixed-wing UAV. The estimated position of the target is then used for the intervention task described in \cite{Fausto}.
If the intervention task requires more precise location of the vessel, the UAV can fly closer to it and keep the vessel in view by performing the implemented visual servo-based approach.
% From the moment the target vessel is detected, the estimated position of the vessel is sent through the communication channel to the USV at the starting gate and it triggers it to start navigating towards provided location \cite{Fausto}.
 \begin{figure}
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[trim = {0 0 3cm 1cm}, clip, width=\textwidth]{images/B}
         \caption{Vessel B}
         \label{fig:VB}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[trim = {3cm 1cm 0 0}, clip, width=\textwidth]{images/D}
         \caption{Vessel D}
         \label{fig:VD}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[trim = {0 0 3cm 1cm}, clip,width=\textwidth]{images/E}
         \caption{Vessel E}
         \label{fig:VE}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[trim = {3cm 1cm 0 0}, clip, width=\textwidth]{images/G}
         \caption{Vessel G}
         \label{fig:VG}
     \end{subfigure}
        \caption{Examples of detected vessels by the front camera of a fixed-wing UAV. Vessel names and detection confidences are highlighted.}
        \label{fig:Vess_example}
\end{figure}

==> Content/extended_abstarct/4-results.tex <==
%results

The proposed approach is validated in the Gazebo-based simulator provided by the organizers using the Robot Operating System (ROS2).
Results include detailed analysis of search pattern selection and successful modeling of velocity based on the angular velocity of the propellers. 
The detection algorithm is tested in a large number of cases and setups. After exhaustive analysis, the detection algorithm showed satisfactory behavior for a fixed-wing UAV flying at an altitude of 100 $m$. At this altitude, the UAV has a wider field of view from the camera and therefore a shorter coverage time. Furthermore, the vessel is detected early enough that the fixed-wing UAV can approach the vessel directly if required. The detection algorithm proved to be robust to the velocity of the fixed-wing UAV, which allowed us to increase the velocity limits to ensure faster execution of the search.
In the full paper, we will go into more detail and provide mathematical explanations for each of the previously mentioned segments, such as fixed-wing UAV control, localization, search, coverage, vessel detection, visual servo control and communication with base station.
